First Searches for Optical Counterparts to Gravitational-wave Candidate Events

During the LIGO and Virgo joint science runs in 2009-2010, gravitational wave (GW) data from three interferometer detectors were analyzed within minutes to select GW candidate events and infer their apparent sky positions. Target coordinates were transmitted to several telescopes for follow-up observations aimed at the detection of an associated optical transient. Images were obtained for eight such GW candidates. We present the methods used to analyze the image data as well as the transient search results. No optical transient was identified with a convincing association with any of these candidates, and none of the GW triggers showed strong evidence for being astrophysical in nature. We compare the sensitivities of these observations to several model light curves from possible sources of interest, and discuss prospects for future joint GW-optical observations of this type.

==> instructions.tex <==
\section{Instructions and good practice}

Use \texttt{Scratch.tex} to leave notes for yourself and your fellow authors.

\begin{figure}
\includegraphics[width=0.50\columnwidth]{test-figure}
\label{fig:test}
\caption{this is a example} 
\end{figure}

\begin{itemize}
\item Use an appropriate prefix for your labels (eq:, fig:, tab:, etc.).
\item Wrap lines to less than 80 characters so we can do diffs between versions.
\item Avoid blank lines following equations in the \LaTeX source, otherwise you
start a new paragraph.  
\item For figures, you should be able to omit the file extension in the
includegraphics\{\} command.  This lets your personal \LaTeX system chose the
preferred format if multiple types are available (e.g., my TeXShop program only
likes PDFs). 
\end{itemize}




==> scratch.tex <==
\section{Scratch}


The \emph{Palomar Transient Factory} (PTF) \cite{PTF2,PTF} operates a 7.3 square
degree FOV camera mounted on the 1.2 m Oschin Telescope at Palomar Observatory.
A typical 60 s exposure detects objects with a limiting magnitude $R=20.5$.  For
the autumn observing period, the PTF team devoted ten fields over several nights
at a target rate of 1 trigger for every three weeks.

\emph{Pi of the Sky} \cite{piofsky} observed using a camera with a 400 square
degree FOV and exposures to limiting magnitude 11--12.  It was located in
Koczargi Stare, near Warsaw.  The camera was a prototype for a planned system
that will simultaneously image two steradians of sky.  The target rate was
approximately 1 per week in the autumn run, followed up with hundreds of 10 s
exposures over several nights.

The \emph{QUEST} camera \cite{quest}, currently mounted on the 1 m ESO Schmidt
Telescope at La Silla Observatory, views 9.4 square degrees of sky in each
exposure. The telescope is capable of viewing to a limiting magnitude of
$R\sim20$.  The QUEST team devoted twelve 60 s exposures over several nights for
each trigger in both the winter and autumn periods, with a target rate of 1
trigger per week.

\emph{ROTSE III} \cite{rotse} is a collection of four robotic telescopes spread
around the world, each with a 0.45 m aperture and 3.4 square degree FOV.  No
filters are used, so the spectral response is that of the CCDs, spanning roughly
400 to 900 nm.  The equivalent $R$ band limiting magnitude is about 17 in a 20 s
exposure.  The ROTSE team arranged for a series of thirty images for the first
night, and several images on following nights, for each autumn run trigger, with
a target rate of 1 trigger per week.

\emph{SkyMapper} \cite{skymap} is a survey telescope located at Siding Spring
observatory in Australia.  The mosaic camera covers 5.7 square degrees of sky in
each field, and is mounted on a 1.35 m telescope with a collecting area
equivalent to an unobscured 1.01 m aperture.  It is designed to reach a limiting
magnitude $g \sim 21$ ($>$$7$ sigma) in a 110 s exposure.  SkyMapper accepted
triggers in the autumn run with a target rate of 1 per week, with several fields
collected for each trigger.

\emph{TAROT} \cite{tarot} operates two robotic 25 cm telescopes, one at La Silla
in Chile and one in Calern, France.  Like the ROTSE III system, each TAROT
instrument has a 3.4 square degree FOV.  A 180 second image with TAROT in ideal
conditions has a limiting $R$ magnitude of $17.5$.  During the winter run, TAROT
observed a single field during one night for each trigger.  In the autumn run,
the field selected for each trigger was observed over several nights.  TAROT
accepted triggers with a target rate of 1 per week.

\emph{Zadko Telescope} \cite{zadko} is a 1 m telescope located in Western
Australia.  The current CCD imager observes fields of 0.15 square degrees down
to magnitude $\sim20$ in the $R$ band for a typical 180 s exposure.  For each
accepted trigger in the autumn run, Zadko repeatedly observed the five galaxies
considered most likely to host the source over several nights.  The target
trigger rate for Zadko was one trigger per week.

The \emph{Liverpool telescope} \cite{liverpool} is a 2 m robotic telescope
situated at the Observatorio del Roque de Los Muchachos on La Palma. For this
project the RATCam instrument, with a 21 square arcminute field of view, was
used.  This instrumentation allows a one hour exposure to reach magnitude
$r'=21$.  This project was awarded 8 hours of target-of-opportunity time, which
was split into 8 observations of 1 hour each, with a target rate of 1 trigger
per week.

